Adapting Pre-trained Generative Models for Extractive Question Answering

Pre-trained Generative models such as BART, T5, etc. have gained prominence as a preferred method for text generation in various natural language processing tasks, including abstractive long-form question answering (QA) and summarization. However, the potential of generative models in extractive QA tasks, where discriminative models are commonly employed, remains largely unexplored. Discriminative models often encounter challenges associated with label sparsity, particularly when only a small portion of the context contains the answer. The challenge is more pronounced for multi-span answers. In this work, we introduce a novel approach that uses the power of pre-trained generative models to address extractive QA tasks by generating indexes corresponding to context tokens or sentences that form part of the answer. Through comprehensive evaluations on multiple extractive QA datasets, including MultiSpanQA, BioASQ, MASHQA, and WikiQA, we demonstrate the superior performance of our proposed approach compared to existing state-of-the-art models.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this work, we propose a new approach for extractive question-answering based on generating indexes of answer tokens or sentences by fine-tuning a pre-trained seq2seq language model. Due to the different kinds of sparsity of labels, discriminative models require dataset-specific customization to achieve good performance in such tasks. We show that generative models can be easily adapted to handle this issue by generating the indexes of the tokens rather than generating the tokens directly. Empirically, our proposed model outperforms specialized state-of-the-art baselines across diverse extractive QA benchmark datasets.


\section{Limitations}
While we have discussed the novelty and importance of our task and the strengths of our proposed approach, here we discuss a few limitations. Generative encoders and decoders such as BART have length restrictions on the input and output sequence.
The input restriction makes it difficult to accommodate very long contexts.
While we have restricted the length in this paper, better solutions are needed in the future.

One limitation of using token-level indexing for multi-span factoid questions is that it uses a lot of extra information to represent the context as we need to insert the index for each token in the context. This is a disadvantage in the scenario where we have a limitation of context length for large language models.

% Applying few-shot instruction-tuned models such as Flan-T5 to this task is difficult due to their token limit. We could have given the context with indexes to Flan-T5 and ask the model to give indexes as answer. But due to the larger context length and additional index tokens, we are exceeding their token limit length most of the cases even with 1/2 examples.  

% Our work does not have any obvious risks.

\section{Ethics Statement}

Our work does not have any ethical issues or obvious risks.



==> experiments_new.tex <==
\section{Experiments}

\subsection{Datasets \& Evaluation Metrics}

To demonstrate the effectiveness of our proposed model for both factoid and long-form question answering, we conducted experiments on multiple extractive QA datasets. Given that our Seq2Seq model generates a sequence as output, we specifically selected datasets that encompass multiple spans as answers. For factoid answer extraction, we utilized the \textbf{MultiSpanQA} dataset \cite{multispanqa_factoid} and the \textbf{BioASQ} dataset \cite{yoon2022sequence} for our experiments. Notably, the \textbf{MultiSpanQA} dataset exclusively comprises multi-span answers and does not include any single-span answers. Furthermore, we also employed the \textbf{BioASQ7b} and \textbf{BioASQ8b} datasets, which serve as benchmarks for biomedical question answering. These datasets focus on list-type questions with multiple extractive factoid answers, providing a comprehensive evaluation environment.

To address long-form question answering, we incorporated the \textbf{MASHQA} dataset \cite{mashqa} from the medical domain into our evaluation. In this dataset, each answer consists of one or more sentences extracted from the context. However, it is important to note that these answer sentences may not be contiguous within the context. Additionally, we utilized the \textbf{WikiQA} dataset \cite{wikiqa}, which focuses on sentence-level extractive question answering. In this dataset, each question is associated with a single-sentence answer. 

For a comprehensive understanding of the datasets used in our experiments, we provide detailed statistics in Appendix Table \ref{data_statistics}. Moreover, to capture the answer sparsity characteristics of these datasets, we present the corresponding information in Appendix Table \ref{tab:sparsity_stat}. As the BART model has a token capacity limit of 1,024, there were instances where we needed to trim the context to ensure it fits within this constraint. The process of context trimming is discussed in Appendix \ref{app:ctx_trm}, providing insights into how we managed the context length.

In accordance with the guidelines provided in the respective dataset papers, we adopted specific evaluation metrics for our experiments. For the sentence-level question answering datasets, MASHQA and WikiQA, we employed sentence-level precision, recall, and F1 score to assess performance. Conversely, for the BioASQ dataset, which operates at the token level, we utilized token-level precision, recall, and F1 score as evaluation metrics. Notably, the MultiSpanQA dataset required a slightly different evaluation approach. In this case, we reported precision, recall, and F1 score based on both exact match (EM) and partial match (PM) criteria to capture the intricacies of the dataset's multi-span answer format.

\subsection{Baseline Models}

To establish baselines, we employed multiple pre-trained language models, namely \textbf{BERT} \cite{devlin2018bert}, \textbf{RoBERTa} \cite{roberta}, \textbf{BioBERT} \cite{lee2020biobert}, \textbf{PubMedBERT} \cite{pubmedbert}, and \textbf{XLNet} \cite{xlnet}, in our experiments. For the task of extracting multi-span factoid answers, we augmented these models with a `BIO' tagging head. For sentence-level extraction, we utilized a sentence classifier head.

In addition to these baselines, we fine-tuned a BART-base \cite{bart} seq2seq model, referred to as {\bf BART\_T}, which directly generates the token sequence as the answer. To evaluate the generated answers under the extractive paradigm, we linked them back to the corresponding context sentences (see Appendix \ref{app:link_back} for further details).

We also incorporated \textbf{MultiCo} \cite{mashqa}, a sentence-level classification model that encodes question and context pairs using XLNet \cite{xlnet}. It classifies each context sentence as either part of the answer or not, utilizing sparsified inter-sentence attention to obtain weights over other context sentences.

As a few-shot baseline, we employed the \textbf{Flan-T5} large model \cite{Chung2022ScalingIL} with eight examples. However, while attempting to generate indexes using this model, we found it to be unsuccessful. Consequently, we directly generated the answer in the few-shot setting for factoid answers. For sentence-level answers, we mapped the generated answer back to the corresponding context sentences (see Appendix \ref{app:link_back} for further details).

Lastly, we leveraged \textbf{LIQUID} \cite{Lee2023LIQUIDAF}, an answer generation framework that utilizes unlabelled corpora to generate high-quality synthetic datasets for various QA tasks. By fine-tuning RoBERTa-base or RoBERTa-large \cite{roberta} with a `BIO' tagging head on both the synthetic dataset and task-specific dataset, LIQUID achieves state-of-the-art performance on the MultiSpanQA and BioASQ datasets.

==> introduction.tex <==
\section{Introduction}

Extractive question-answering task is solved mainly using discriminative models. For datasets with single-span factoid answers like SQuAD \cite{squad}, models like \cite{zhang2021retrospective, yamada2020luke, zhang2020sg} find the start and end of the answer span. For datasets with multi-span factoid answers such as MultiSpanQA \cite{multispanqa_factoid}, BioASQ \cite{yoon2022sequence}, `BIO' tagging based discriminative models are proposed. For long-form sentence-level QA datasets like MASHQA \cite{mashqa} or WikiQA \cite{wikiqa}, sentence classification models are used \cite{mashqa}. But we have not seen any seq2seq models to solve this extractive QA task.

% Extractive question-answering is an important task in NLP. In addition to works on factoid question answering \cite{roberta, xlnet,squad,squad2,msmarco,searchqa,triviaqa} where answers have shorter span, long-form QA has gained popularity recently \cite{khashabi2021gooaq, krishna2021hurdles, asqa, ilfqa}, and many datasets have been made public in this area \cite{google_nq,eli5,wikiqa}. Discriminative models are mostly proposed to solve this task. Seq2Seq models are explored extensively for abstractive long-form QA, but they have hardly been used for extractive QA tasks. 

% , this idea may not work in a straightforward manner as models need to find multiple spans of the answer. So for datasets like MultiSpanQA \cite{multispanqa_factoid} or BioASQ \cite{yoon2022sequence}, `BIO' based tagging models are used. Here models assign `BI' tags to different parts of the answers and assign `O' tags to the non-answer tokens. 

We observe that in the case of extractive QA, answers contain a very small fraction of the tokens or sentences in the given context (see \ref{app:sparsity_stat}). For the single-span answers, this sparsity is not an issue as models focus on finding the start and end of the answer span. The loss function does not involve the non-answer part of the context. But for multi-span answers where `BIO' tagging is used, models suffer from sparsity problems as large number of non-answer tokens are assigned `O' tags. A similar challenge will be there for sentence-level extractive QA datasets like MASHQA \cite{mashqa} where answer sentences are spread across multiple spans. State-of-the-art answer extraction models, such as MultiCo \cite{mashqa}, uses the sentence selection method to find the answer sentences. Since answers can be of multiple sentences spread across multiple spans, they use binary classification for each sentence in the context. Such discriminative sentence selection models struggle with the sparsity of the answer with respect to the context. 

This sparsity is less of a challenge for generative approaches since these only explicitly model what is likely and not what is unlikely.
Additionally, large pre-trained generative seq2seq models have been shown to perform excellently in many tasks in recent years \cite{rebel, retrieve_gen}. 
However, the application of generative seq2seq models for an extractive task brings up two questions.
What should the model generate, and  does this make the task harder than necessary?
We address these two issues by proposing to {\em generate the indexes of context tokens or sentences} which are part of the extractive answer.
This uses the generative approach while significantly restricting the output space so that it is easier to learn a distribution over it.
The training burden is also reduced by fine-tuning large pre-trained models. 
We are not aware of any prior work using direct generation via seq2seq models for extractive question answering.
We show that this generative approach outperforms state-of-the-art answer extraction models. 
One of the main strengths of our proposed approach is that it is simple and applicable to any multi-span extractive task.
We evaluate our proposed approach on five extractive QA datasets and show that it outperforms the state-of-the-art which are often customized models for specific datasets\footnote{We will release our code and data upon acceptance.}. 

% Our proposed model works for tasks as diverse as token-level multi-span answer extraction to and multi-span and single-span factoid answer extraction.

% To summarize, our contributions are as follows:
% (1) We propose a simple, yet very effective approach to adapt the generative seq2seq models for multi-span answer extraction in a general-purpose fashion.
% (2) We show that our proposed approach outperforms state-of-the-art answer extraction models not only for technical question answering but also for multi-span answer extraction tasks from multiple domains. 


\begin{table*}[t]
\small
\centering
\begin{tabular}{{p{0.95\textwidth}}}
\hline

{\bf Question}: What happens during a clinical trial for arthritis treatment? \\ \hline
{\bf Context}: \\
\textbf{1} \textcolor{red}{A clinical trial is a research study conducted with patients to evaluate a new arthritis treatment, drug, or device.} \\
\textbf{2} {The purpose of clinical trials is to find new and improved methods of treating arthritis.} \\
\textbf{3} {Clinical trials make it possible to apply the latest scientific and technological advances in arthritis to patient care.} \\
\textbf{4} \textcolor{red}{During a clinical trial, doctors use the best available arthritis treatment as a standard to evaluate new treatments.} \\
\textbf{5} \textcolor{red} {The new treatments are considered to be at least as effective or possibly more effective than the standard.} \\
\textbf{6} {New treatment options are first researched in a laboratory where they are carefully studied in the test tube and in animals.} \\
\textbf{7} \textcolor{red} {Only the treatments most likely to work are further evaluated in a small group of humans prior to applying them in a larger clinical trial. }\\
\textbf{8} {When a new arthritis treatment is studied for the first time in humans, it is not known exactly how it will work.} \\
\ldots \\
\textbf{17} {The researchers determine the best way to give the new treatment and how much of it can be given safely.} \\
\textbf{18} {Phase II clinical trials determine the effect of the research treatment on patients and usually the best dosage.} \\ \ldots
\\ \hline
{\bf Extracted Answer as Full Index (FI) Sequence}: 1 4 5 7 \\ %\hline
{\bf Extracted Answer as Span Index (SI) Sequence}: (1 1) (4 5) (7 7) \\ \hline                          
\end{tabular}
\caption{Illustration of the task of extracting reference answers from MASH-QA. Example of context, multi-span extractive answer, and two different representations of it using sentence indexes. For the index span sequence, each pair denotes begin and end indexes of the span. Sentence indexes are shown in bold, answer sentences in red, and parentheses are added for span index sequence for ease of illustration. }
\label{tab:example}
\end{table*}

==> results.tex <==
\section{Experimental Results}

First, we experiment with QA datasets having short spans as answers such as MultiSpanQA and BioASQ and include the performance in Table \ref{tab:multispanqa} and \ref{tab:bioasq}. We see that our proposed full index sequence generation and span index sequence generation both works equally well on these datasets. Our BART\_FI$_l$ model achieves 1\% higher F1 score than the LIQUID model \cite{Lee2023LIQUIDAF} on partial match-based F1 score. On the BioASQ8b dataset, our BART\_SI$_l$ and BART\_FI$_l$ models achieve new SOTA performance that is 3\% higher then previous SOTA LIQUID$\_l$ model. On BioASQ7b dataset as well, our model achieves very close to the SOTA performance of LIQUID$\_l$. 

% Experiments on these three short answer span datasets show that our proposed model works equally well on this QA task along with long-form QA task.

\begin{table}[ht]
\centering
\small
\begin{tabular}{l|ccc|ccc}
\hline
 & \multicolumn{3}{c|}{Exact Match} & \multicolumn{3}{c}{Partial Match}  \\ \hline
 Model & P & R & F1 & P & R & F1 \\ \hline
 FLAN-T5 & 0.45 & 0.23 & 0.30 & 0.72 & 0.53 & 0.61  \\ 
BERT$_b$ & 0.58 & 0.61 & 0.59 & 0.80 & 0.73 & 0.76 \\
BART\_T$_b$ & 0.59 & 0.61 & 0.60 & 0.80 & 0.77 & 0.78 \\ 
% BigBERTa$_l$* & 0.71 & 0.75 & 0.73 & 0.86 & 0.88 & \textbf{0.87} \\
% SpanQualifier* & 0.72 & 0.73 & 0.73 & 0.85 & 0.85 & 0.85  \\ 
LIQUID$_b$ & 0.66 & 0.69 & 0.67 & 0.81 & 0.81 & 0.81  \\ 
LIQUID$_l$ & 0.75 & 0.68 & \textbf{0.71} & 0.85 & 0.77 & 0.81 \\ \hline 
BART\_SI$_b$ & 0.62 & 0.61 & 0.61 & 0.79 & 0.75 & 0.77  \\
BART\_FI$_b$ & 0.61 & 0.62 & 0.61 & 0.78 & 0.76 & 0.77 \\
BART\_SI$_l$ & 0.67 & 0.69 & 0.68 & 0.81 & 0.82 & 0.81  \\
BART\_FI$_l$ & 0.66 & 0.70 & 0.68 & 0.80 & 0.85 & \textbf{0.82}  \\ \hline

\end{tabular}%
\caption{Performance comparison of our proposed model against the SOTA baselines on MultiSpanQA.}
\label{tab:multispanqa}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[ht]
\small
\begin{tabular}{l|lll|lll}
\hline
                            & \multicolumn{3}{c|}{BioASQ7b} & \multicolumn{3}{c}{BioASQ8b} \\ \hline
Model                       & P        & R        & F1       & P        & R       & F1       \\ \hline
FLAN-T5                & 0.23     & 0.45     & 0.31    & 0.16     & 0.40    & 0.23    \\
BART\_T$_b$  & 0.25     & 0.41     & 0.31    & 0.22     & 0.41    & 0.29    \\ 
BioBERT & 0.42     & 0.58     & 0.45    & 0.39     & 0.59    & 0.44    \\
% BlueBERT                & 0.40     & 0.62     & 0.45    & 0.34     & 0.57    & 0.39    \\ 
PMBERT & 0.43     & 0.63     & 0.48    & 0.38     & 0.59    & 0.43    \\
LIQUID$_b$ & 0.41     & 0.61     & 0.49    & 0.37     & 0.56    & 0.44    \\
LIQUID$_l$  & 0.45     & 0.64     & \textbf{0.53}    & 0.39     & 0.59    & 0.47    \\ \hline
BART\_SI$_b$              & 0.44     & 0.55     & 0.49    & 0.43     & 0.51    & 0.46    \\ 
BART\_FI$_b$               & 0.43     & 0.57     & 0.49    & 0.42     & 0.51    & 0.46    \\
BART\_SI$_l$                & 0.48     & 0.57     & 0.52    & 0.47     & 0.54    & \textbf{0.50}    \\ 
BART\_FI$_l$                & 0.47     & 0.57     & 0.52    & 0.45     & 0.55    & \textbf{0.50}    \\
\hline
\end{tabular}%
\caption{Performance comparison of our proposed method against the SOTA baselines on BioASQ 7b and 8b datasets. PMBERT refers to PubMedBERT.}
\label{tab:bioasq}
\end{table}

Next, we experiment with sentence-level long-form QA datasets MASHQA and WikiQA and include the results in Table \ref{tab:mashqa_wikiqa}. On MASHQA, our BART-large models (BART\_SI$_l$ and BART\_FI$_l$) achieve a 2\% higher F1 score than the previous SOTA XLNet model. On the WikiQA dataset, our BART-large models achieve a 3\% higher F1 score than the previous SOTA Flan-T5 model. These results show that our proposed adaption of the pre-trained Seq2Seq language models outperforms the baselines on the sentence-level answer extraction task without any task-specific modifications in the model. 

\begin{table}[ht]
\small
\begin{tabular}{l|lll|lll}
\hline
Model        & \multicolumn{3}{c|}{MASHQA} & \multicolumn{3}{c}{WikiQA} \\ \hline
             & P        & R       & F1      & P       & R       & F1     \\ \hline
BERT         & 0.42     & 0.63    & 0.50     & 0.48    & 0.56    & 0.52   \\
RoBERTa      & 0.48     & 0.62    & 0.54    & 0.56    & 0.54    & 0.55   \\
XLNet        & 0.61     & 0.74    & 0.67    & 0.49    & 0.51    & 0.50    \\
MultiCo      & 0.61     & 0.73    & 0.66    & 0.57    & 0.57    & 0.57   \\
BART\_{T}$_b$       & 0.59     & 0.32    & 0.41    & 0.47    & 0.35    & 0.40    \\ 
FLAN-T5  & 0.62     & 0.22    & 0.33    & 0.68     & 0.68     & 0.68    \\ \hline
BART\_SI$_b$ & 0.68     & 0.69    & 0.68    & 0.63    & 0.63     & 0.63    \\ 
BART\_FI$_b$  & 0.66     & 0.71    & 0.68    & 0.64    & 0.64     & 0.64   \\
BART\_SI$_l$ & 0.64     & 0.74    &\textbf{0.69}    & 0.71     & 0.71    & \textbf{0.71}    \\ 
BART\_FI$_l$  & 0.63     & 0.76    & \textbf{0.69}    & 0.71     & 0.71     & \textbf{0.71}    \\ \hline

\end{tabular}%
\caption{Performance comparison of our proposed model against SOTA baselines on MASH-QA and WikiQA in terms of sentence level Precision, Recall and F1 scores.}
\label{tab:mashqa_wikiqa}
\end{table}

% \textbf{*} indicates that results are statistically significant ($p<0.05$ as measured by paired T-test)



In summary, the above experimental results provide clear evidence that the index sequence generation approach is able to outperform specialized state-of-the-art models across diverse extractive QA tasks and datasets with no task-specific customization. Previous SOTA models do not perform uniformly across the five datasets. Our proposed model perform equally well in all these datasets which shows the generalization capability of the the model.



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

In Table \ref{tab:ablation}, we include the ablation of our model. As we do not use much sophistication on the BART model itself, the only ablation we can think of is removing the index tokens from the context and then generating the answer indexes. From Table \ref{tab:ablation}, we see BART-base or BART-large models perform almost equally well or badly on these five datasets. The plausible reason is that both these models do not understand the meaning of the output sequence without their presence in the context. Now if we compare these results against the numbers in Table \ref{tab:mashqa_wikiqa}, \ref{tab:multispanqa}, \ref{tab:bioasq}, we see that adding those index numbers in the context greatly improves the performance of the BART-base and BART-large models.

% Particularly on the BioASQ datasets, BART performs very poorly when index numbers are removed from the context. One plausible reason could be that these BioASQ datasets are from the biomedical domain which is different from the training data domains of BART. 


\begin{table}[ht]
\small
\centering
\begin{tabular}{l|c|c}
\hline
            & BART\_FI$_b$ & BART\_FI$_l$ \\ \hline
MASHQA      & 0.63   & 0.64   \\ 
WikiQA      & 0.37   & 0.36   \\ 
MultiSpanQA & 0.52   & 0.53   \\ 
BioASQ7b    & 0.05   & 0.06   \\ 
BioASQ8b    & 0.06   & 0.07   \\ \hline
\end{tabular}
\caption{F1 scores of our proposed model without using sentence or token index in the input context. For MultiSpanQA, we report the partial match F1 score here.}
\label{tab:ablation}
\end{table}







% \subsection{Analysis}

% \textbf{Analysis on MASH-QA: }

% We have done two types of analysis on the answer extraction output a) Performance of the answer extraction engine with an answer length and b) Performance of the answer extraction engine with an answer span.

% \textbf{Performance of the Answer Extraction Engine with an Answer length: }

% \begin{figure}[ht]
% \includegraphics[width=\columnwidth]{prec_rec_vs_ans_len1.png}
% \caption{Performance of answer extraction with variation in answer length (in terms of the number of sentences in the answer).}
% \label{pre_rec_ans_len}
% \centering
% \end{figure}

% Fig.~\ref{pre_rec_ans_len} depicts the performance of the best-performing answer extraction model $BART\_si\_span$ with the length of an answer. We observe that the precision of answer extraction increases and recall decreases with the length of the answer. The reason being for a long answer the sentences that the answer extraction engine retrieves are correct but it fails to retrieve all correct answer sentences whereas, for a short answer, it is just the opposite. One simple explanation of these could be that since the average length of answers in our data set is around three sentences so for short answers it retrieves some extra sentences and for long answers, it retrieves a few sentences.

% \textbf{Performance of the answer extraction engine with an answer span}

% \begin{figure}[ht]
% \includegraphics[width=\columnwidth]{answer_span.png}
% \caption{Performance of answer extraction with variation in answer length (in terms of the number of sentences in the answer).}
% \label{ans_span}
% \centering
% \end{figure}

% Fig.~\ref{ans_span} shows that the best-performing answer extraction engine $BART\_si\_span$ works better with single-span answers.

% \begin{table*}[ht]
% \centering
% \small
% \begin{tabular}{l|llllll|llllll}
%  &
%   \multicolumn{6}{c|}{MultiSpanQA} &
%   \multicolumn{6}{c}{MultiSpanQAE} \\ \hline
%  &
%   \multicolumn{3}{c|}{Exact Match} &
%   \multicolumn{3}{c|}{Partial Match} &
%   \multicolumn{3}{c|}{Exact Match} &
%   \multicolumn{3}{c}{Partial Match} \\ \hline
%  Model & P & R & \multicolumn{1}{l|}{F1} &
%   P &
%   R &
%   F1 &
%   P &
%   R &
%   \multicolumn{1}{l|}{F1} &
%   P &
%   R &
%   F1 \\ \hline
% BERT$_b$ &
%   0.58 &
%   0.61 &
%   \multicolumn{1}{l|}{0.59} &
%   0.80 &
%   0.73 &
%   0.76 &
%   0.43 &
%   0.42 &
%   \multicolumn{1}{l|}{0.42} &
%   0.74 &
%   0.68 &
%   0.70 \\ 
%   BigBERTa$_l$* &
%   0.71 &
%   0.75 &
%   \multicolumn{1}{l|}{0.73} &
%   0.86 &
%   0.88 &
%   \textbf{0.87} &
%   - &
%   - &
%   \multicolumn{1}{l|}{-} &
%   - &
%   - &
%   - \\
% SpanQualifier* &
%   0.72 &
%   0.73 &
%   \multicolumn{1}{l|}{0.73} &
%   0.85 &
%   0.85 &
%   0.85 &
%   0.69 &
%   0.73 &
%   \multicolumn{1}{l|}{0.71} &
%   0.81 &
%   0.83 &
%   \textbf{0.82} \\ 
%   LIQUID$_b$ &
%   0.66 &
%   0.69 &
%   \multicolumn{1}{l|}{0.67} &
%   0.81 &
%   0.81 &
%   0.81 &
%   - &
%   - &
%   \multicolumn{1}{l|}{-} &
%   - &
%   - &
%   - \\ 
%   LIQUID$_l$ &
%   0.75 &
%   0.68 &
%   \multicolumn{1}{l|}{0.71} &
%   0.85 &
%   0.77 &
%   0.81 &
%    - &
%    - &
%   \multicolumn{1}{l|}{-} &
%    - &
%    - &
%    - \\ \hline 
%   BART\_SI$_b$&
%   0.62 &
%   0.61 &
%   \multicolumn{1}{l|}{0.61} &
%   0.79 &
%   0.75 &
%   0.77 &
%   0.59 &
%   0.58 &
%   \multicolumn{1}{l|}{0.58} &
%   0.70 &
%   0.72 &
%   0.71 \\
%   BART\_FI$_b$&
%   0.61 &
%   0.62 &
%   \multicolumn{1}{l|}{0.61} &
%   0.78 &
%   0.76 &
%   0.77 &
%   0.60 &
%   0.61 &
%   \multicolumn{1}{l|}{0.61} &
%   0.74 &
%   0.73 &
%   0.73 \\
% BART\_SI$_l$ &
%   0.67 &
%   0.69 &
%   \multicolumn{1}{l|}{0.68} &
%   0.81 &
%   0.82 &
%   0.81 &
%   0.61 &
%   0.68 &
%   \multicolumn{1}{l|}{0.64} &
%   0.74 &
%   0.80 &
%   0.77 \\
% BART\_FI$_l$ &
%   0.66 &
%   0.70 &
%   \multicolumn{1}{l|}{0.68} &
%   0.80 &
%   0.85 &
%   0.82 &
%   0.61 &
%   0.70 &
%   \multicolumn{1}{l|}{0.65} &
%   0.74 &
%   0.82 &
%   0.78 \\
%   \hline
% \end{tabular}%
% \caption{Performance comparison of our proposed model against the SOTA baselines on MultiSpanQA and MultiSpanQAE. * marked baselines are unpublished works taken from MultiSpanQA leaderboard.}
% \label{tab:multispanqa}
% \end{table*}
